StyleTTS 2: Towards Human-Level Text-to-Speech through Style Diffusion and Adversarial Training with Large Speech Language Models

In this paper, we present StyleTTS 2, a text-to-speech (TTS) model that leverages style diffusion and adversarial training with large speech language models (SLMs) to achieve human-level TTS synthesis. StyleTTS 2 differs from its predecessor by modeling styles as a latent random variable through diffusion models to generate the most suitable style for the text without requiring reference speech, achieving efficient latent diffusion while benefiting from the diverse speech synthesis offered by diffusion models. Furthermore, we employ large pre-trained SLMs, such as WavLM, as discriminators with our novel differentiable duration modeling for end-to-end training, resulting in improved speech naturalness. StyleTTS 2 surpasses human recordings on the single-speaker LJSpeech dataset and matches it on the multispeaker VCTK dataset as judged by native English speakers. Moreover, when trained on the LibriTTS dataset, our model outperforms previous publicly available models for zero-shot speaker adaptation. This work achieves the first human-level TTS on both single and multispeaker datasets, showcasing the potential of style diffusion and adversarial training with large SLMs. The audio demos and source code are available at https://styletts2.github.io/.

==> methods.tex <==
%auto-ignore

\subsection{StyleTTS Overview}

\label{sec:3.1}
StyleTTS \cite{li2022styletts} is a non-autoregressive TTS framework using a style encoder to derive a style vector from reference audio, enabling   natural and expressive speech generation. The style vector is incorporated into the decoder and duration and prosody predictors using adaptive instance normalization (AdaIN) \cite{huang2017arbitrary}, allowing the model to generate speech with varying duration, prosody, and emotions.

The model comprises eight modules, organized into three categories: (1) a speech generation system (acoustic modules) with a text encoder, style encoder, and speech decoder; (2) a TTS prediction system with duration and prosody predictors; and (3) a utility system for training, including a discriminator, text aligner, and pitch extractor (see Appendix \ref{app:F} for detailed descriptions). It undergoes a two-stage training process: the first stage trains the acoustic modules for mel-spectrogram reconstruction, and the second trains TTS prediction modules using the fixed acoustic modules trained in the first stage.

In the first stage, the text encoder $T$ encodes input phonemes $\bm{t}$ into phoneme representations $\bm{h}_{\text{text}} = T(\bm{t})$, while the text aligner $A$ extracts speech-phoneme alignment $\bm{a}_\text{algn} = A(\bm{x}, \bm{t})$  from input speech $\textbf{x}$ and phonemes $\bm{t}$ to produce aligned phoneme representations $\bm{h}_\text{algn} = \bm{h}_\text{text} \cdot \bm{a}_\text{algn}$ via dot product. Concurrently, the style encoder $E$ obtains the style vector $\bm{s} = E(\textbf{x})$, and the pitch extractor $F$ extracts the pitch curve $p_{\bm{x}} = F(\bm{x})$ along with its energy $n_{\bm{x}} = \norm{\bm{x}}$. Lastly, the speech decoder $G$ reconstructs $\hat{\bm{x}} = G\parn{\bm{h}_\text{algn}, \bm{s}, p_{\bm{x}}, n_{\bm{x}}}$, which is trained to match input $\bm{x}$ using a $L_1$ reconstruction loss $\mathcal{L}_\text{mel}$ and adversarial objectives $\mathcal{L}_\text{adv}, \mathcal{L}_\text{fm}$ with a discriminator $D$. Transferable monotonic aligner (TMA) objectives are also applied to learn optimal alignments (see Appendix \ref{app:G} for details).

In the second stage, all components except the discriminator $D$ are fixed, with only the duration and prosody predictors being trained. The duration predictor $S$ predicts the phoneme duration with $\bm{d}_\text{pred} = S(\bm{h}_{\text{text}}, \textbf{s})$, whereas the prosody predictor $P$ predicts pitch and energy as $\hat{p}_{\bm{x}}, \hat{n}_{\bm{x}} = P(\bm{h}_{\text{text}}, \bm{s})$. The predicted duration is trained to match the ground truth duration $\bm{d}_\text{gt}$ derived from the summed monotonic version of the alignment $\bm{a}_\text{algn}$ along the time axis with an $L_1$ loss $\mathcal{L}_\text{dur}$. The predicted pitch $\hat{p}_{\bm{x}}$ and energy $\hat{n}_{\bm{x}}$ are trained to match the ground truth pitch $p_{\bm{x}}$ and energy $n_{\bm{x}}$ derived from pitch extractor $F$ with $L_1$ loss $\mathcal{L}_{f0}$ and $\mathcal{L}_{n}$. During inference, $\bm{d}_\text{pred}$ is used to upsample $\bm{h}_\text{text}$ through $\bm{a}_\text{pred}$, the predicted alignment, obtained by repeating the value 1 for $\bm{d}_{\text{pred}}[i]$ times at $\ell_{i-1}$, where $\ell_{i}$ is the end position of the $i^\text{th}$ phoneme $\bm{t}_i$ calculated by summing $\bm{d}_{\text{pred}}[k]$ for $k \in \{1, \ldots, i\}$, and $\bm{h}_\text{text}[i]$ and $\bm{d}_{\text{pred}}[i]$ are the representation and predicted duration of $\bm{t}_i$. The mel-spectrogram is synthesized by $\bm{x}_\text{pred} = G(\bm{h}_{\text{text}} \cdot \bm{a}_\text{pred}, S(\bm{\tilde{x}}), \hat{p}_{\bm{\tilde{x}}}, \hat{n}_{\bm{\tilde{x}}})$ with $\bm{\tilde{x}}$ an arbitrary reference audio that influences the style of $\bm{x}_\text{pred}$, which is then converted into a waveform using a pre-trained vocoder. 

% Despite its state-of-the-art performance in synthesizing diverse, controllable speech through reference audio, StyleTTS has several drawbacks. Firstly, the model's two-stage training process, with an additional vocoding stage, complicates training and negatively impacts high-quality speech synthesis due to the covariate shift between the acoustic models, predictors, and vocoders. Secondly, the deterministic nature of the model means it always generates the same audio given the same reference speech, limiting its expressiveness and capability to address the one-to-many problem in TTS synthesis. Lastly, the model's reliance on reference speech for generation makes it less suitable for real-time applications where reference audio may not always be readily available.

Despite its state-of-the-art performance in synthesizing diverse and controllable speech, StyleTTS has several drawbacks, such as a two-stage training process with an additional vocoding stage that degrades sample quality, limited expressiveness due to deterministic generation, and reliance on reference speech hindering real-time applications.

\subsection{StyleTTS 2} 

\begin{figure}[!t]

\vspace{-10 pt}
  \centering
  \subfigure[Acoustic modules pre-training and joint training. To accelerate training, the pre-training first optimize modules inside the blue box; the joint training then follows to optimize all components except the pitch extractor, which is used to provide the ground truth label for pitch curves. The duration predictor is trained with only $\mathcal{L}_\text{dur}$. ]{\includegraphics[width=\textwidth]{figure/Fig1a_2tmp_1.pdf}}
  \subfigure[SLM adversarial training and inference. WavLM is pre-trained and not tuned. Unlike (a), the duration predictor is trained E2E with all components with $\mathcal{L}_{slm}$ (eq. \ref{eq:celoss}) via differentiable upsampling. ]{\includegraphics[width=0.9\textwidth]{figure/Fig1b_2_1.pdf}}
  \vspace{-5 pt}
  \caption{Training and inference scheme of StyleTTS 2.}
  \vspace{-8 pt}
\label{fig:1}

\end{figure}

StyleTTS 2 improves upon the StyleTTS framework, resulting in a more expressive text-to-speech (TTS) synthesis model with human-level quality and improved out-of-distribution performance. We introduce an end-to-end (E2E) training process that jointly optimizes all components, along with direct waveform synthesis and adversarial training with large speech language models (SLMs) enabled by our innovative differentiable duration modeling. The speech style is modeled as a latent variable sampled through diffusion models, allowing diverse speech generation without reference audio. We outline these important changes in the following sections with an overview in Figure \ref{fig:1}.

\subsubsection{End-to-End Training} 
\label{sub:3.2.2}
E2E training optimizes all TTS system components for inference without relying on any fixed components like pre-trained vocoders that convert mel-spectrograms into waveforms \cite{kim2021conditional, lim2022jets}. To achieve this, we modify the decoder $G$ to directly generate the waveform from the style vector, aligned phoneme representations, and pitch and energy curves. We remove the last projection layer for mel-spectrograms of the decoder and append a waveform decoder after it. We propose two types of decoders: HifiGAN-based and iSTFTNet-based. The first is based on Hifi-GAN \cite{kong2020hifi}, which directly generates the waveform. In contrast, the iSTFTNet-based decoder \cite{kaneko2022istftnet} produces magnitude and phase, which are converted into waveforms using inverse short-time Fourier transform for faster training and inference. We employ the snake activation function \cite{ziyin2020neural}, proven effective for waveform generation in \cite{lee2022bigvgan}. An AdaIN module \cite{huang2017arbitrary} is added after each activation function to model the style dependence of the speech, similar to the original StyleTTS decoder. We replace the mel-discriminator in \cite{li2022styletts} with the multi-period discriminator (MPD) \cite{kong2020hifi} and multi-resolution discriminator (MRD) \cite{jang2021univnet} along with the LSGAN loss functions \cite{mao2017least} for decoder training, and incorporate the truncated pointwise relativistic loss function \cite{li2022improve} to enhance sound quality (see Appendix \ref{app:F} and \ref{app:G} for details).
 
To accelerate training, before jointly optimizing all components, we first pre-train the acoustic modules along with the pitch extractor and text aligner via $\mathcal{L}_\text{mel}, \mathcal{L}_\text{adv}, \mathcal{L}_\text{fm}$ and TMA objectives for $N$ epochs where $N$ depends on the size of the training set, in the same way as the first training stage of \cite{li2022styletts}. We then jointly optimize $\mathcal{L}_\text{mel}, \mathcal{L}_\text{adv}, \mathcal{L}_\text{fm}, \mathcal{L}_\text{dur}, \mathcal{L}_\text{f0}$ and $\mathcal{L}_\text{n}$, where $\mathcal{L}_\text{mel}$ is modified to match the mel-spectrograms of waveforms reconstructed from predicted pitch $\hat{p}_{\bm{x}}$ and energy $\hat{n}_{\bm{x}}$  (Fig \ref{fig:1}a).  During joint training, stability issues emerge from diverging gradients, as the style encoder must encode both acoustic and prosodic information. To address this inconsistency, we introduce a \textit{prosodic} style encoder $E_{p}$ alongside the original \textit{acoustic} style encoder $E_{a}$, previously denoted as $E$ in section \ref{sec:3.1}. Instead of using $\bm{s}_a = E_a(\bm{x})$, predictors $S$ and $P$ take $\bm{s}_p = E_p(\bm{x})$ as the input style vector. The style diffusion model generates the augmented style vector $\bm{s} = [\bm{s}_p, \bm{s}_d]$. This modification effectively improves sample quality (see section \ref{sec:5.3}). To further decouple the acoustic modules and predictors, we replace the phoneme representations $\bm{h}_\text{text}$ from $T$, now referred to as \textit{acoustic} text encoder, with $\bm{h}_\text{bert}$ from another text encoder $B$ based on BERT transformers, denoted as \textit{prosodic} text encoder. Specifically, we employ a phoneme-level BERT \cite{li2023phoneme} pre-trained on extensive corpora of Wikipedia articles as the prosodic text encoder. This approach has been shown to enhance the naturalness of StyleTTS in the second training stage \cite{li2023phoneme} , similar to our proposed usage here. % $B$ are jointly trained with $G, S, P, E_a$, and $E_p$.

With differentiable upsampling and fast style diffusion, we can generate speech samples during training in a fully differentiable manner, just as during inference. These samples are used to optimize  $\mathcal{L}_{slm}$ (eq. \ref{eq:celoss}) during joint training to update the parameters of all components for inference (Fig \ref{fig:1}b).  

\subsubsection{Style Diffusion}
\label{sub:3.2.1}
In StyleTTS 2, we model the speech $\bm{x}$ as a conditional distribution  $p(\bm{x}|\bm{t}) = \int p(\bm{x}|\bm{t}, \bm{s})p(\bm{s}|\bm{t})\,d\bm{s}$ through a latent variable $\bm{s}$ that follows the distribution $p(\bm{s}|\bm{t})$. We call this variable  the \textit{generalized speech style}, representing any characteristic in speech beyond phonetic content $\bm{t}$, including but not limited to prosody, lexical stress, formant transitions, and speaking rate \cite{li2022styletts}. We sample $\bm{s}$ by EDM \cite{karras2022elucidating} that follows the combined probability flow \cite{huang2021variational} and time-varying Langevin dynamics \cite{song2020score}:

\begin{equation}
\label{eq:score}
    \bm{s} = \int -\sigma(\tau)\left[\beta(\tau)\sigma(\tau) + \dot{\sigma}(\tau)\right]\nabla_{\bm{s}} \log p_{\tau}(\bm{s}|\bm{t})\,d\tau + \int \sqrt{2\beta(\tau)}\sigma(\tau)\,d\tilde{W}_\tau,
\end{equation}
where $\sigma(\tau)$ is the noise level schedule and $\dot{\sigma}(\tau)$ is its time derivative, $\beta(\tau)$ is the stochasticity term, $\tilde{W}_\tau$ is the backward Wiener process for $\tau \in [{T}, 0]$ and $\nabla_{\bm{s}}\log p_{\tau}(\bm{s}|\bm{t})$ is the score function at time $\tau$. 

% \begin{equation}
% \label{eq:score}
%     \bm{s}(t) = \int [a(\bm{s}, t) - g(t)^2\nabla_{\bm{s}}\log p_{t}(\bm{s}|\bm{t})]\,dt + \int g(t)\,d\tilde{W}_t
% \end{equation}
% where $a(\cdot, t)$ is the drift coefficient, $g(t)
% $ is the diffusion coefficient, $\tilde{W}_t$ is the backward Wiener process for $t \in [{T}, 0]$ and $\nabla_{\bm{s}}\log p_{t}(\bm{s}|\bm{t})]$ is score function of $p(\bm{s}|\bm{t})$ at the diffusion process time $t$. 

We follow the EDM \cite{karras2022elucidating} formulation with the denoiser $K(\bm{s}; \bm{t}, \sigma)$ preconditioned as:

\begin{equation}
\label{eq:edm}
    K(\bm{s}; \bm{t}, \sigma) := \parn{\frac{\sigma_\text{data}}{\sigma^*}}^2\bm{s} + \frac{\sigma \cdot \sigma_\text{data}}{\sigma^*} \cdot V\parn{\frac{\bm{s}}{\sigma^*}; \bm{t}, \frac{1}{4}\ln\sigma},
\end{equation}
where $\sigma$ follows a log-normal distribution $\ln \sigma \sim \mathcal{N}(P_{\text{mean}}, P_{\text{std}}^2)$ with $P_{\text{mean}} = -1.2$, $P_{\text{std}} = 1.2$, $\sigma^* := \sqrt{\sigma^2 + \sigma_{\text{data}}^2}$ is the scaling term, $\sigma_{\text{data}} = 0.2$ is the empirical estimate of the standard deviation of style vectors, and $V$ is a 3-layer transformer \cite{vaswani2017attention} conditioned on $\bm{t}$ and $\sigma$ which is trained with:
\begin{equation}
\label{eq:edmloss}
    \mathcal{L}_\text{edm} = \mathbb{E}_{\bm{x}, \bm{t}, \sigma, \bm{\xi} \sim \mathcal{N}(0, I)}\left[\lambda(\sigma) \norm{K(\bm{E}(\bm{x}) + \sigma\bm{\xi}; \bm{t}, \sigma) - \bm{E}(\bm{x})}_2^2\right],
\end{equation}
where $\bm{E}(\bm{x}) := [E_a(\bm{x}), E_p(\bm{x})]$, and $\lambda(\sigma) := (\sigma^*/(\sigma \cdot \sigma_{\text{data}}))^2$ is the weighting factor. Under this framework, equation \ref{eq:score} becomes an ODE where the score function depends on $\sigma$ instead of $\tau$: 
\begin{equation}
\label{eq:ode}
    \frac{d\bm{s}}{d\sigma} = -\sigma \nabla_{\bm{s}}\log p_{\sigma}(\bm{s}|\bm{t}) = \frac{\bm{s} - K(\bm{s}; \bm{t}, \sigma)}{\sigma}, \hspace{5mm} \bm{s}(\sigma(T)) \sim \mathcal{N}(0, \sigma(T)^2I).
\end{equation}
Unlike \cite{karras2022elucidating} that uses 2nd-order Heun, we solve eq. \ref{eq:ode} with the ancestral DPM-2 solver \cite{lu2022dpm} for fast and diverse sampling as we demand speed more than accuracy. On the other hand, we use the same scheduler as in \cite{karras2022elucidating} with $\sigma_{\text{min}} = 0.0001, \sigma_{\text{max}} = 3$ and $\rho = 9$. This combination allows us to sample a style vector for high-quality speech synthesis with only three steps, equivalent to running a 9-layer transformer model, minimally impacting the inference speed (see Appendix \ref{app:B} for more discussions).  

$V$ conditions on $\bm{t}$ through $\bm{h}_\text{bert}$ concatenated with the noisy input ${\bm{E}(\bm{x}) + \sigma\xi}$, and $\sigma$ is conditioned via sinusoidal positional embeddings \cite{vaswani2017attention}. In the multispeaker  setting, we model $p(\bm{s}|\bm{t}, \bm{c})$ by $K(\bm{s};\bm{t}, \bm{c}, \sigma)$ with the additional speaker embedding $\bm{c} = \bm{E}(\bm{x}_\text{ref})$ where $\bm{x}_\text{ref}$ is the reference audio of the target speaker. The speaker embedding $\bm{c}$ is injected into $V$ by adaptive layer normalization \cite{li2022styletts}. 
  
\subsubsection{SLM Discriminators}
\label{sub:3.2.4}
Speech language models (SLMs) encode valuable information ranging from acoustic to semantic aspects \cite{pasad2021layer}, and SLM representations are shown to mimic human perception for evaluating synthesized speech quality \cite{kaneko2022istftnet}. % Our experiments also demonstrate that a simple linear probe with SLM representations can classify human recordings or generated speech with over 90\% accuracy (see Appendix \ref{app:C}). Inspired by these findings, we use SLMs as discriminators, being the first to transfer knowledge from SLM encoders to generative tasks via adversarial training.
We uniquely transfer knowledge from SLM encoders to generative tasks via adversarial training by employing a 12-layer WavLM \cite{chen2022wavlm} pre-trained on 94k hours of data \footnote{Available at \url{https://huggingface.co/microsoft/wavlm-base-plus}} as the discriminator. 
%To prevent the discriminator from overpowering the generator due to the larger number of parameters in SLMs
As the number of parameters of WavLM is greater than StyleTTS 2, to avoid discriminator overpowering, we fix the pre-trained WavLM model $W$ and append a convolutional neural network (CNN) $C$ as the discriminative head. We denote the SLM discriminator $D_{SLM} = C \circ W$. The input audios are downsampled to 16 kHz before being fed into $D_{SLM}$ to match that of WavLM. $C$ pools features $\bm{h}_\text{SLM} = W(\bm{x})$ from all layers with a linear map from $13 \times 768$ to 256 channels. We train the generator components ($T, B, G, S, P, V$, denoted as $\bm{G}$) and $D_{SLM}$ to optimize:

\begin{equation}
\label{eq:celoss}
     \mathcal{L}_{slm} = \min\limits_{\bm{G}}\max\limits_{D_{SLM}} \parn{\mathbb{E}_{\bm{x}} [\log D_{SLM}(\bm{x})] + \mathbb{E}_{\bm{t}} [\log \parn{1 - D_{SLM}(\bm{G}(\bm{t}))}]},
\end{equation}
where $\bm{G}(\bm{t})$ is the generated speech with text $\bm{t}$, and $\bm{x}$ is the human recording. 
\cite{sauer2021projected} shows that:
\begin{equation}
    D^*_{SLM}(\bm{x}) = \frac{\mathbb{P}_{W \circ \mathcal{T}} (\bm{x})}{\mathbb{P}_{W \circ \mathcal{T}} (\bm{x}) + \mathbb{P}_{W \circ \mathcal{G}} (\bm{x})},
\end{equation}
where $D^*_{SLM}(\bm{x})$ is the optimal discriminator, $\mathcal{T}$ and $\mathcal{G}$ represent true and generated data distributions, while $\mathbb{P}_\mathcal{T}$ and $\mathbb{P}_\mathcal{G}$ are their respective densities. The optimal $\bm{G}^*$ is achieved if $\mathbb{P}_{W \circ \mathcal{T}} = \mathbb{P}_{W \circ \mathcal{G}}$, meaning that when converged, $\bm{G}^*$ matches the generated and true distributions in the SLM representation space, effectively mimicking human perception to achieve human-like speech synthesis.

In equation \ref{eq:celoss}, the generator loss is independent of ground truth $\bm{x}$ and relies only on input text $\bm{t}$. This enables training on out-of-distribution (OOD) texts, which we show in section \ref{sec:5.3} can improve the performance on OOD texts. In practice, to prevent $D_{SLM}$ from over-fitting on the content of the speech, we sample in-distribution and OOD texts with equal probability during training.


\subsubsection{Differentiable Duration Modeling}
\label{sub:3.2.3}

The duration predictor produces phoneme durations $\bm{d}_\text{pred}$, but the upsampling method described in section \ref{sec:3.1} to obtain $\bm{a}_\text{pred}$ is not differentiable, blocking gradient flow for E2E training. NaturalSpeech \cite{tan2022naturalspeech} employs an attention-based upsampler \cite{elias2021parallel} for human-level TTS. However, we find this approach unstable during adversarial training because we train our model using differentiable upsampling with only the adversarial objective described in eq. \ref{eq:celoss} and without extra loss terms due to the length mismatch caused by  deviations of $\bm{d}_{\text{pred}}$ from $\bm{d}_{\text{gt}}$. Although this mismatch can be mitigated with soft dynamic time warping as used in \cite{elias2021parallel, tan2022naturalspeech}, we find this approach both computationally expensive and unstable with mel-reconstruction and adversarial objectives. To achieve human-level performance with adversarial training, a non-parametric upsampling method is preferred for stable training.

Gaussian upsampling \cite{donahue2020end} is non-parametric and  converts the predicted duration $\bm{d}_\text{pred}$ into $\bm{a}_\text{pred}[n, i]$ using a Gaussian kernel $\mathcal{N}_{c_i}(n; \sigma)$ centered at $c_i := \ell_i - \frac{1}{2}\bm{d}_\text{pred}[i]$ with the hyperparameter $\sigma$:

\setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}

\begin{minipage}{.6\linewidth}
\begin{equation}
\label{eq:rbf}
    \mathcal{N}_{c_i}(n;\sigma) := \exp\parn{-\frac{(n - c_i)^2}{2\sigma^2}},
\end{equation}
\end{minipage}%
\begin{minipage}{.4\linewidth}
\begin{equation}
    \ell_i := \sum\limits_{k=1}^i \bm{d}_\text{pred}[k],
  \label{eq:ell}
\end{equation}
\end{minipage}

where $\ell_i$ is the end position and $c_i$ is the center position of the $i^\text{th}$ phoneme $\bm{t}_i$. However, Gaussian upsampling has limitations due to its fixed width of Gaussian kernels determined by $\sigma$. This constraint prevents it from accurately modeling alignments with varying lengths depending on $\bm{d}_\text{pred}$. Non-attentive Tacotron \cite{shen2020non} extends this by making $\sigma_i$ trainable, but the trained parameters introduce instability for E2E training with adversarial loss, similar to issues of attention-based upsamplers.

We propose a new non-parametric differentiable upsampler without additional training while taking into account the varying length of the alignment. For each phoneme $\bm{t}_i$, we model the alignment as a random variable $a_i \in \mathbb{N}$, indicating the index of the speech frame the phoneme $\bm{t}_i$ is aligned with. We define the duration of the $i^\text{th}$ phoneme as another random variable $d_i \in \{1, \ldots, L\}$, where $L = 50$ is the maximum phoneme duration hyperparameter, equivalent to 1.25 seconds in our setting. We observe that $a_i = \sum\limits_{k=1}^i d_k$, but each $d_k$ is dependent on each other, making the sum difficult to model. Instead, we approximate $a_i = d_i + \ell_{i-1}$. The approximated probability mass function (PMF) of $a_i$ is

\setlength{\belowdisplayskip}{0pt} \setlength{\belowdisplayshortskip}{0pt}
\setlength{\abovedisplayskip}{0pt} \setlength{\abovedisplayshortskip}{0pt}
\begin{equation}
\label{eq:pmf}
    f_{a_i}[n] = f_{d_i + \ell_{i-1}}[n]  = f_{d_i}[n]  * f_{\ell_{i-1}}[n]  = \sum\limits_k f_{d_i}[n] \cdot \delta_{\ell_{i-1}}[n - k],
\end{equation}

where $\delta_{\ell_{i-1}}$ is the PMF of $\ell_{i-1}$, a constant defined in eq. \ref{eq:ell}. This Kronecker delta function is not differentiable, so we replace it with $\mathcal{N}_{\ell_{i-1}}$ defined in eq. \ref{eq:rbf} with $\sigma = 1.5$ for sufficient gradient flow. % which we found to be sufficiently large for the gradient flow while keeping it as close to $\delta_{\ell_i}$ as possible. 

To model $f_{d_i}$, we modify the duration predictor to output $q[k, i]$, the probability of the $i^\text{th}$ phoneme having a duration of at least $k$ for $k \in \{1, \ldots, L\}$, optimized to be 1 when $\bm{d}_\text{gt} \geq k$ with the cross-entropy loss  (see Appendix \ref{app:G}). Under this new scheme, we can approximate $\bm{d}_\text{pred}[i] := \sum\limits_{k=1}^L q[k, i]$, trained to match $\bm{d}_\text{gt}$ with $\mathcal{L}_\text{dur}$ as in section \ref{sec:3.1}. The vector $q[:, i]$ can be viewed as the unnormalized version of $f_{d_i}$, though it is trained to be uniformly distributed across the interval $[1, d_i]$. Since the number of speech frames $M$ is usually larger than the number of input phonemes $N$, this uniform distribution aligns single phonemes to multiple speech frames as desired. Finally, we normalize the differentiable approximation $\tilde{f}_{a_i}[n]$ across the phoneme axis, as in \cite{donahue2020end}, to obtain $\bm{a}_\text{pred}$ using the softmax function:
\begin{minipage}{.45\linewidth}
\begin{equation}
    \bm{a}_\text{pred}[n, i] := \frac{e^{\parn{\tilde{f}_{a_i}[n]})}}{\sum\limits_{i=1}^N e^{\parn{\tilde{f}_{a_i}[n]}}}, 
  \label{eq:apred}
\end{equation}
\end{minipage}%
\begin{minipage}{.55\linewidth}
\begin{equation}
    \tilde{f}_{a_i}[n] := \sum\limits_{k = 0}^{\hat{M} }q[n, i] \cdot \mathcal{N}_{\ell_{i-1}}(n - k; \sigma),
  \label{eq:tildef}
\end{equation}
\end{minipage}
where $\hat{M} := \left\lceil\ell_N\right\rceil$ is the predicted total duration of the speech and $n \in \{1, \ldots, \hat{M}\}$. An illustration of our proposed differentiable duration modeling is given in Figure \ref{fig:4} (Appendix \ref{app:C}). 
